Just Add $100 More: Augmenting NeRF-based Pseudo-LiDAR Point Cloud for Resolving Class-imbalance Problem

Typical LiDAR-based 3D object detection models are trained in a supervised manner with real-world data collection, which is often imbalanced over classes (or long-tailed). To deal with it, augmenting minority-class examples by sampling ground truth (GT) LiDAR points from a database and pasting them into a scene of interest is often used, but challenges still remain: inflexibility in locating GT samples and limited sample diversity. In this work, we propose to leverage pseudo-LiDAR point clouds generated (at a low cost) from videos capturing a surround view of miniatures or real-world objects of minor classes. Our method, called Pseudo Ground Truth Augmentation (PGT-Aug), consists of three main steps: (i) volumetric 3D instance reconstruction using a 2D-to-3D view synthesis model, (ii) object-level domain alignment with LiDAR intensity estimation and (iii) a hybrid context-aware placement method from ground and map information. We demonstrate the superiority and generality of our method through performance improvements in extensive experiments conducted on three popular benchmarks, i.e., nuScenes, KITTI, and Lyft, especially for the datasets with large domain gaps captured by different LiDAR configurations. Our code and data will be publicly available upon publication.

==> figs/fig_hungarian.tex <==
\begin{figure}[h]
    \begin{center}
    \includegraphics[width=1\linewidth]{assets/hungarian.png}
    \end{center}
    \vspace{-1em}
    \caption{\textbf{Illustrations of Ball Patch Matching.} We patchify both the source domain point cloud and the target domain point cloud with an equal number of patches using the ball query operator. We find optimal matching between ball patches by leveraging Hungarian matching based on their center distances.}
    \label{fig:hungarian}
    \vspace{-1em}
\end{figure}

==> figs/fig_nusc_trainval.tex <==
\begin{figure}[h]
    \centering
    \caption{\textbf{nuScenes Long-tail Class Distribution}}\label{fig:nusctrainval}
    \includegraphics[width=1\linewidth]{assets/nusc_trainval.png}
\end{figure}

==> figs/fig_radiance.tex <==
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=0.7\linewidth]{assets/radiance_short.png}
    \end{center}
    \vspace{-1em}
    \caption{\textbf{Volumetric 3D Instance Rendering Results.} (a) Examples of our data collection: (i) a set of images capturing miniatures from different views and (ii) public videos of certain minor-class objects. (b) We use a 2D-to-3D renderer to convert different view images into a 3D volumetric representation.}\label{fig:radiance}
    \vspace{-1em}
\end{figure}

==> figs/stats_combine.tex <==

%\setlength{\tabcolsep}{4pt}
% \renewcommand{\arraystretch}{0.8}
\begin{figure}[t]
  \begin{minipage}[t]{.5\linewidth}
    \centering
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1}


    \captionof{table}{\textbf{Mixing ratio between GT and PGT objects}}\label{tab:mixing}
    \resizebox{\linewidth}{!}{\begin{tabular}{@{}lcccccc|c}
        \toprule
        \small{Data Source} & \small{C.V} & \small{Trailer} & \small{Truck} & \small{Bus} & \small{M.C} & \small{B.C} & Total\\
        \midrule \midrule
        \small{Miniatures} & 10 & 4 & 5 & 3 & 6 & 3 & 31\\
        \small{Public Videos} & 2 & - & 64 & 10 & 21 & - & 97 \\
        \bottomrule
    \end{tabular}
    }
  \end{minipage}
  % \hspace{1em}
  
\end{figure}
%Bus & 17.7 & 13.1 & \textbf{13.0} & 13.2 & 8.7 & 19.8  \\
%Construction Vehicle & \textbf{7.0} & 7.6 & 7.5 & 7.6 & - & 6.0 \\
%Trailer & 20.6 & 11.9 & \textbf{11.9} & 12.2 & -  & 36.5 \\
%Truck & 8.9 & 7.6 & 7.6 & \textbf{7.3} & 6.6  & 13.4  \\
%Motorcycle & 20.7 & 7.0 & 7.2 & \textbf{3.7} & 3.0  & 10.1 \\
%Bicycle & 9.0 & 2.2 & 2.4 & \textbf{2.1} & 1.8  & 0.7 \\
%\midrule

==> tables/abl_fid_map.tex <==
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1}
\begin{table}[t]
    \centering
    \caption{\textbf{Downstream Performance on FID scores.} mAP scores and NDS scores comparison between variants of generated banks and public LiDAR datasets, Lyft~\cite{DBLP:conf/corl/HoustonZBYCJOIO20} and A2D2~\cite{DBLP:journals/corr/abs-2004-06320}. Abbr. G.S: Gaussian Splatting} \label{tab:abl_fid_map}
    \vspace{-1em}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|rrrrr|r|rr}
    \toprule 
    & \multicolumn{6}{c|}{Pseudo-LiDAR Point Clouds} & Lyft~\cite{DBLP:conf/corl/HoustonZBYCJOIO20} & A2D2~\cite{DBLP:journals/corr/abs-2004-06320} \\
    \midrule
    Volumetric 3D type & \multicolumn{5}{c|}{Plenoxel~\cite{DBLP:conf/cvpr/Fridovich-KeilY22}} & G.S~\cite{DBLP:journals/tog/KerblKLD23} & - & - \\
    \hline
    Azimuth Resolution (px) & $3600$ & $1080$ &$1080$ & $1080$ & $1080$ & $1080$ & - & - \\
    RGB features & \cmark & \xmark & \xmark & \cmark & \cmark & \cmark & - & - \\
    Group intensity Loss & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & - & - \\
    \hline
    \# of samples & \multicolumn{6}{c|}{136K} & 37K & 11K\\
    \midrule 
    \midrule 
    Avg. FID Score ($\downarrow$) & 14.2 & 8.2 & 8.3 & 8.3 & \textbf{7.7} & \textbf{7.1} & 4.8 & 14.4 \\
    \hline
    mAP ($\uparrow$) & 63.40 & 63.44 & 63.48 & 63.41 & \textbf{63.52} & &  63.45 & 63.17 \\ 
    NDS ($\uparrow$) & 68.83 & 68.99 & 69.02 & 68.87 & \textbf{69.11} &  & 68.88 & 68.73\\
    \bottomrule
    \end{tabular}}
    % \vspace{-2em}
\end{table}

==> tables/auc.tex <==
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.3}
\begin{table}[t]
    \centering
    \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule
    Model & A & B & C & D & E & F \\\midrule
    Random Placement~\cite{DBLP:journals/sensors/YanML18} & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark\\
    Ground-based Placement~\cite{DBLP:journals/corr/abs-2305-12853}  & \xmark & \xmark & \cmark & \cmark & \cmark &  \cmark \\
    Map-based Placement & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark 
     \\\midrule
    w/ Pseudo LiDAR Augmentation & \xmark & \cmark & \xmark & \cmark & \xmark & \cmark\\
    \midrule \midrule
    Bus & 85.8 & 85.9 & 86.5 & 86.6 & 87.0 & 86.7 \\
    Construction Vehicle & 43.7 & 43.3 & 51.3 & 52.1 & 52.4 & 52.7 \\
    Trailer & 61.0 & 61.9 & 67.2 & 67.0 & 68.4 & 66.3 \\
    Truck & 71.7 & 73.0 & 72.9 & 73.3 & 74.0 & 74.8 \\
    Motorcycle & 68.5 & 69.7 & 74.7 & 75.1 & 75.6 & 77.3 \\
    Bicycle & 50.5 & 53.5 & 61.7 & 63.3 & 63.3 & 64.2 \\
    \bottomrule
    \end{tabular}}
    \caption{\textbf{Precision-Recall Area under Curve (PR AUC) of tail classes on nuScene \textit{val} set.} $^\dagger$: our reproduction.}
    \label{tab:auc}
\end{table}

==> tables/fid_downstream.tex <==
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1}
\begin{table}[t]
    \centering
    \caption{\textbf{Quality of Pseudo LiDAR Point Clouds.} FID scores (squared Wasserstein distance between given samples and true nuScenes samples, thus lower is better) comparison between variants of our models and public LiDAR datasets, Lyft~\cite{DBLP:conf/corl/HoustonZBYCJOIO20} and A2D2~\cite{DBLP:journals/corr/abs-2004-06320}. Abbr. G.S: Gaussian Splatting}  
    \vspace{-1em}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lrrrrr|r|rr}
    \toprule 
    & \multicolumn{6}{c|}{Our Pseudo-LiDAR Point Clouds} & Lyft~\cite{DBLP:conf/corl/HoustonZBYCJOIO20} & A2D2~\cite{DBLP:journals/corr/abs-2004-06320} \\
    \midrule
    Volumetric 3D type & \multicolumn{5}{c|}{Plenoxel} & G.S & - & - \\
    \hline
    Azimuth Resolution (px) & $3600$ & $1080$ &$1080$ & $1080$ & $1080$ & $1080$ & - & - \\
    RGB features & \cmark & \xmark & \xmark & \cmark & \cmark & \cmark & - & - \\
    Group intensity Loss & \cmark & \xmark & \cmark & \xmark & \cmark & \cmark & - & - \\
    \hline
    \# of samples & \multicolumn{6}{c|}{136K} & 37K & 11K\\
    \hline
    % \midrule 
    Bus & 17.7 & 14.6 & 13.1 & \textbf{13.0} & 13.2 & 10.8 & 8.7 & 19.8  \\
    Construction Vehicle & \textbf{7.0} & 7.5 & 7.6 & 7.5 & 7.6 & 7.6 & - & 6.0 \\
    Trailer & 20.6 & 12.7 & 11.9 & \textbf{11.9} & 12.2 & 13.8 & -  & 36.5 \\
    Truck & 8.9 & 8.4 & 7.6 & 7.6 & \textbf{7.3} & 6.8 & 6.6 & 13.4  \\
    Motorcycle & 20.7 & 2.5 & 7.0 & 7.2 & \textbf{3.7} & 1.1 & 3.0  & 10.1 \\
    Bicycle & 9.0 & 3.3 & 2.2 & 2.4 & \textbf{2.1} & 2.0 & 1.8 & 0.7 \\
    \midrule
    Avg. FID Score ($\downarrow$) & 14.2 & 8.2 & 8.3 & 8.3 & \textbf{7.7} & 7.0 & 4.8 & 14.4 \\
    \hline
    mAP ($\uparrow$) & 63.40 & 63.44 & 63.48 & 63.41 & \textbf{63.52} & &  63.45 & 63.17 \\ 
    NDS ($\uparrow$) & 68.83 & 68.99 & 69.02 & 68.87 & \textbf{69.11} &  & 68.88 & 68.73\\
    \bottomrule
    \end{tabular}}
    \label{tab:fid}
    % \vspace{-1em}
\end{table}

==> tables/fid_variance.tex <==

\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\begin{table}[h]
    \centering
    \vspace{-1.5em}
    \caption{\textbf{Detection performance on various LiDAR samples.}}
    \vspace{-1em}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|rrrrr|rr}
    \toprule 
    Azimuth Res. (px) & $3600$ & $1080$ & $1080$ & $1080$ & $1080$ & \multirow{2}{*}{Lyft} & \multirow{2}{*}{A2D2}\\
    RGB / Group Loss & \cmark/\cmark & \xmark/\xmark & \xmark/\cmark & \cmark/\xmark & \cmark/\cmark & &  \\
    \midrule \midrule
    \# of samples & \multicolumn{5}{c|}{136K} & 37K & 11K\\
    \hline
    FID ($\downarrow$) & 14.2 & 8.2 & 8.3 & 8.3 & \textbf{7.7} & 4.8 & 14.4 \\
    \hline
    mAP ($\uparrow$) & 63.40 & 63.44 & 63.48 & 63.41 & \textbf{63.52} & 63.45 & 63.17 \\ 
    NDS ($\uparrow$) & 68.83 & 68.99 & 69.02 & 68.87 & \textbf{69.11} & 68.88 & 68.73\\
    \bottomrule
    \end{tabular}}
    \vspace{-1em}
    \label{tab:rebuttal_fid}
\end{table}

%Bus & 17.7 & 13.1 & \textbf{13.0} & 13.2 & 8.7 & 19.8  \\
%Construction Vehicle & \textbf{7.0} & 7.6 & 7.5 & 7.6 & - & 6.0 \\
%Trailer & 20.6 & 11.9 & \textbf{11.9} & 12.2 & -  & 36.5 \\
%Truck & 8.9 & 7.6 & 7.6 & \textbf{7.3} & 6.6  & 13.4  \\
%Motorcycle & 20.7 & 7.0 & 7.2 & \textbf{3.7} & 3.0  & 10.1 \\
%Bicycle & 9.0 & 2.2 & 2.4 & \textbf{2.1} & 1.8  & 0.7 \\
%\midrule


==> tables/other.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lrr}
\toprule 
& Lyft & A2D2 \\
\midrule \midrule
mAP ($\uparrow$) &  &  \\ 
NDS ($\uparrow$) &  &  \\
\bottomrule
\end{tabular}
    \caption{\textbf{Quality of Pseudo LiDAR Point Clouds.} mAP and NDS scores comparison between variants of our models and public LiDAR datasets, Lyft and A2D2.}\label{tab:rebuttal_other}
    % \vspace{-1em} 
\end{table}

%Bus & 17.7 & 13.1 & \textbf{13.0} & 13.2 & 8.7 & 19.8  \\
%Construction Vehicle & \textbf{7.0} & 7.6 & 7.5 & 7.6 & - & 6.0 \\
%Trailer & 20.6 & 11.9 & \textbf{11.9} & 12.2 & -  & 36.5 \\
%Truck & 8.9 & 7.6 & 7.6 & \textbf{7.3} & 6.6  & 13.4  \\
%Motorcycle & 20.7 & 7.0 & 7.2 & \textbf{3.7} & 3.0  & 10.1 \\
%Bicycle & 9.0 & 2.2 & 2.4 & \textbf{2.1} & 1.8  & 0.7 \\
%\midrule


==> tables/size.tex <==
\begin{table}[t]
    \centering
    \caption{Continuously increasing pseudo-LiDAR data}\label{tab:rebuttal_bank}
    \vspace{-1em}
    \begin{tabular}{cccc}
    \toprule 
    Size & bank 1/4 & bank 1/2 & Full bank \\
    \midrule \midrule
    mAP ($\uparrow$) & 63.18 & 63.43 & \textbf{63.52} \\ 
    NDS ($\uparrow$) & 68.72 & 68.94 & \textbf{69.11} \\
    \bottomrule
    \end{tabular}
\end{table}

%Bus & 17.7 & 13.1 & \textbf{13.0} & 13.2 & 8.7 & 19.8  \\
%Construction Vehicle & \textbf{7.0} & 7.6 & 7.5 & 7.6 & - & 6.0 \\
%Trailer & 20.6 & 11.9 & \textbf{11.9} & 12.2 & -  & 36.5 \\
%Truck & 8.9 & 7.6 & 7.6 & \textbf{7.3} & 6.6  & 13.4  \\
%Motorcycle & 20.7 & 7.0 & 7.2 & \textbf{3.7} & 3.0  & 10.1 \\
%Bicycle & 9.0 & 2.2 & 2.4 & \textbf{2.1} & 1.8  & 0.7 \\
%\midrule
%\begin{table}[h]
%    \centering
%    \caption{\textbf{Mixing ratio between GT and PGT samples}}
%    \vspace{-1em}
%    \begin{tabular}{cccc}
%    \toprule 
%    Size & 1/4 bank & 1/2 bank & Full bank \\
%    \midrule \midrule
%    mAP ($\uparrow$) &  & 63.43 & 63.52 \\ 
%    NDS ($\uparrow$) &  & 68.94 & 69.11 \\
%    \bottomrule
%    \end{tabular}
%    \label{tab:rebuttal_mixing}
%\end{table}

==> tables/test2.tex <==
%\setlength{\tabcolsep}{4pt}
%\renewcommand{\arraystretch}{1.0}
\begin{table}[t]
    \centering
    \caption{\textbf{Detection performance comparison on nuScenes \textit{test} set in terms of AP, mAP, and NDS}. We use CP-Voxel~\cite{DBLP:conf/cvpr/YinZK21} and Transfusion-L~\cite{DBLP:conf/cvpr/BaiHZHCFT22} as a baseline model. $^\dagger$: our reproduction, $^\ddagger$: test time augmentation enabled.}\label{tab:test}
    \vspace{-1em}    
    \begin{tabular}{l|ccc|ccc}
    \toprule
    %\multirow{2}{*}{Model} & \multicolumn{3}{c|}{CP-Voxel~\cite{DBLP:conf/cvpr/YinZK21}$^\ddagger$} & \multicolumn{3}{c}{Transfusion-L~\cite{DBLP:conf/cvpr/BaiHZHCFT22}} \\\cmidrule{2-7}
    Model & \multicolumn{3}{c|}{CP-Voxel~\cite{DBLP:conf/cvpr/YinZK21}$^\ddagger$} & \multicolumn{3}{c}{Transfusion-L~\cite{DBLP:conf/cvpr/BaiHZHCFT22}} \\
    \hline
    %\cmidrule{2-7}
    % & A & B & C & D & E & F \\\midrule
    %CP-Voxel~\cite{DBLP:conf/cvpr/YinZK21} & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark \\
    %TF-L~\cite{DBLP:conf/cvpr/BaiHZHCFT22} & \xmark & \xmark & \xmark & \cmark & \cmark & \cmark \\ \midrule
    %w/ Test time Augmentation~\cite{} & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark\\
    w/ GT-Aug~\cite{DBLP:journals/sensors/YanML18} & \cmark & \xmark & \xmark & \cmark & \xmark & \xmark \\
    w/ Real-Aug$^\dagger$~\cite{DBLP:journals/corr/abs-2305-12853} & \xmark & \cmark & \xmark & \xmark & \cmark & \xmark \\
    w/ PGT-Aug (ours) & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark\\
    \midrule\midrule
    Bus & 64.4 & 64.5 & \textbf{68.1} & 63.7 & 64.3 & \textbf{67.3}\\
    Construction Vehicle & \textbf{31.0} & 29.0 & 29.0 & 29.0 & \textbf{31.0} & 30.1 \\
    Trailer & 60.0 & 60.1 & \textbf{61.7} & 58.7 & 60.0 & \textbf{60.2}\\
    Truck & 47.2 & 57.3 & \textbf{57.7} & 46.3 & 47.3 & \textbf{56.9} \\
    Motorcycle & 65.7 & 72.2 & \textbf{74.0} & 67.1 & 65.7 & \textbf{68.2} \\
    Bicycle & 41.0 & 47.1 & \textbf{48.6} & 44.2 & 41.0 & \textbf{40.6}\\
    \midrule
    mAP ($\uparrow$, \textit{for all 10 classes}) & 63.8 & 65.8 & \textbf{67.1} & 63.9 & 63.8 & \textbf{65.1}\\
    NDS ($\uparrow$, \textit{for all 10 classes}) & 68.7 & 71.3 & \textbf{72.3} & 68.6 & 68.7 & \textbf{69.9}\\ 
    \bottomrule
    \end{tabular}
\end{table}
%\textbf{Mean Average Precision (mAP) and nuScenes Detection Score (NDS) of CP-Voxel and TF-L on nuScenes \textit{test} set.} $^\dagger$: our reproduction.
